RealDexUMI: A Wearable Universal Manipulation Interface for Dexterous Robot Learning

Learning dexterous manipulation requires demonstrations that preserve fine hand-object interactions while remaining executable at deployment. Existing pipelines either lose deployable dexterity through retargeting or embodiment conversion, or rely on robot-specific teleoperation that is costly to scale and often lacks intuitive, contact-aware control for dexterous data collection. We present RealDexUMI, a wearable universal manipulation interface built around a shared dexterous end-effector module that integrates a lightweight dexterous hand, in-hand vision, and fingertip tactile sensing. A palm-side isomorphic teleoperation glove maps human finger inputs to robot-hand joint commands, enabling real-time, retargeting-free, intuitive, and precise hand control. The shared hand and sensing modules yield zero-gap end-effector data, with matched in-hand observations, tactile signals, contacts, and hand actions between collection and deployment. Across eight real-robot tasks spanning fine-grained, contact-rich, long-horizon, and bimanual manipulation, policies trained on RealDexUMI data achieve an average success rate of 88.75%, generalize to unseen initial poses, and transfer across three embodiments. Website: https://research.beingbeyond.com/realdexumi

==> figures/table_dp.tex <==
```latex
\subsection{Diffusion Policy Baseline}
\label{app:dp_baseline}

We additionally train Diffusion Policy on the same RealDexUMI demonstrations using the same observation and action interface as the ACT policies in the main experiments.
This evaluation tests whether RealDexUMI data can support another common imitation-learning policy backend.

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\caption{
Diffusion Policy success rates across eight real-robot tasks.
Per-task entries report success rates in $[0,1]$ over 20 trials, and Avg. reports the overall success percentage.
}
\label{tab:dp_success}
\begin{tabular}{
L{2.3cm}
C{1.0cm}
C{1.4cm}
C{1.0cm}
C{1.0cm}
C{1.0cm}
C{1.0cm}
C{1.0cm}
C{1.0cm}
C{1.5cm}
}
\toprule
\textbf{Method} 
& \textbf{Cube} 
& \textbf{Multi-obj.} 
& \textbf{Plug} 
& \textbf{Cap} 
& \textbf{Tea} 
& \textbf{Drawer} 
& \textbf{Egg} 
& \textbf{Biman.} 
& \textbf{Avg.} \\
\midrule
Diffusion Policy
& 0.85
& 0.75
& 0.25
& 0.75
& 0.40
& 0.60
& 0.80
& 0.70
& 63.75\% \\
\bottomrule
\end{tabular}
\end{table}
```


==> table_ablation.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{
Selected ablations on contact-rich tasks.
Each result is evaluated over 20 real-robot trials.
}
\label{tab:policy_ablation}
\begin{tabular}{lccc}
\toprule
Policy Variant & Drawer & Plug insertion & Egg carton \\
\midrule
Full RealDexUMI & 17/20 & 17/20 & 14/20 \\
w/o tactile input & --/20 & --/20 & --/20 \\
Hand state as hand action & --/20 & --/20 & --/20 \\
\bottomrule
\end{tabular}
\end{table}

==> table_subgoal.tex <==
\begin{tabular}{llc}
\toprule
Task & Subgoal & Cumulative Completion \\
\midrule
Drawer stowing & Open drawer & 20/20 \\
 & Pick cube & 18/20 \\
 & Close drawer & 17/20 \\
Tea picking & Pick tweezer & 17/20 \\
 & Pick tea & 16/20 \\
 & Place tea in cup & 16/20 \\
Egg handling & Open carton & 15/20 \\
 & Pick egg & 14/20 \\
 & Place egg in pan & 14/20 \\
Multi-object grasping & Grasp first object & 20/20 \\
 & Grasp second object & 20/20 \\
\bottomrule
\end{tabular}
